On the Impacts of Halo Model Implementations in Sunyaev-Zeldovich Cross-Correlation Analyses

Statistical studies of the circumgalactic medium (CGM) using Sunyaev-Zeldovich (SZ) observations offer a promising method of studying the gas properties of galaxies and the astrophysics that govern their evolution. Forward modeling profiles from theory and simulations allows them to be refined directly off of data, but there are currently significant differences between the thermal SZ (tSZ) observations of the CGM and the predicted tSZ signal. While these discrepancies could be inherent, they could also be the result of decisions in the forward modeling used to build statistical measures off of theory. In order to see effects of this, we compare an analysis utilizing halo occupancy distributions (HODs) implemented in halo models to simulate the galaxy distribution against a previous studies which weighted their results off of the CMASS galaxy sample, which contains nearly one million galaxies, mainly centrals of group sized halos, selected for relatively uniform stellar mass across redshifts between $0.4<z<0.7$. We review some of the implementation differences that can account for changes, such as miscentering, one-halo/two-halo cutoff radii, and mass ranges, all of which will need to be given the proper attention in future high-signal-to-noise studies. We find that our more thorough model predicts a signal $\sim 25\%$ stronger than the one from previous studies on the exact same sample, resulting in a $33\%$ improved fit for non-dust-contaminated angular scales. Additionally, we find that modifications that change the satellite fraction even by just a few percents, such as editing the halo mass range and certain HOD parameters, result in strong changes in the final signal. Although significant, this discrepancy from the modeling choices is not large enough to completely account for the existing disagreements between simulations and measurements.

==> makefile <==
# Makefile to produce the article.
LATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: latex
PDFLATEX  = pdflatex -shell-escape 
DVIPS  =  dvips
PSPDF  =  ps2pdf
FIGURES = figures/

.PRECIOUS: $(FIGURES)

default: main.pdf

%.pdf : $(FIGURES) %.tex
	$(PDFLATEX) $*.tex	
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
#	$(DVIPS) -o $*.ps $*.dvi
#	$(PSPDF) $*.ps $*.pdf
	make clean

clean:
	rm -f *.log *.toc *.aux *.bak *.blg *.obj *.out

realclean:
	rm -f *.log *.toc *.aux *.obj *.bak *.bbl *.blg *.brf \
              *~ */*~ *.bak */*.bak 

